Can Large Language Models be Good Emotional Supporter? Mitigating Preference Bias on Emotional Support Conversation

Emotional Support Conversation (ESC) is a task aimed at alleviating individuals' emotional distress through daily conversation. Given its inherent complexity and non-intuitive nature, ESConv dataset incorporates support strategies to facilitate the generation of appropriate responses. Recently, despite the remarkable conversational ability of large language models (LLMs), previous studies have suggested that they often struggle with providing useful emotional support. Hence, this work initially analyzes the results of LLMs on ESConv, revealing challenges in selecting the correct strategy and a notable preference for a specific strategy. Motivated by these, we explore the impact of the inherent preference in LLMs on providing emotional support, and consequently, we observe that exhibiting high preference for specific strategies hinders effective emotional support, aggravating its robustness in predicting the appropriate strategy. Moreover, we conduct a methodological study to offer insights into the necessary approaches for LLMs to serve as proficient emotional supporters. Our findings emphasize that (1) low preference for specific strategies hinders the progress of emotional support, (2) external assistance helps reduce preference bias, and (3) existing LLMs alone cannot become good emotional supporters. These insights suggest promising avenues for future research to enhance the emotional intelligence of LLMs.

==> tab_tex/case_study_llms_1.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l p{10cm}}
    \toprule
    Dialogue Background & The following is a conversation between a supporter and a seeker about depression regarding a/an breakup with partner. The seeker says "\textbf{After breaking up with the partner I had lot of stress and depression in my life. I was facing really a mental stress without my boyfriend.}"  \\
    \midrule
    \multirow{12}{*}{
        \textbf{Dialogue Context}
    }
    & \underline{\textit{seeker}}: How was your day \\
    & \underline{\textit{supporter}}: \textbf{(Others)} Boring\\
    & \underline{\textit{seeker}}: It really very stress full and depressed situation.  \\
    & \underline{\textit{seeker}}: Why your day is boring  \\
    & \underline{\textit{supporter}}: \textbf{(Question)} Don't worry about my day, I'm 34 and retired I do this to help people, tell me about your situation.\\
    & \underline{\textit{seeker}}: My situation is really very sad and depressed \\
    & \underline{\textit{supporter}}: \textbf{(Restatement or Paraphrasing)} I was a homeless drug-addicted junkie for over 10 years. Tell me how yours is worse sweety.\\
    & \underline{\textit{supporter}}: \textbf{(Question)} Tell me why you are so sad and depressed. \\
    & \underline{\textit{seeker}}: I had a breakup with my partner, it was really very horrible for me to overcome. \\
    & \underline{\textit{supporter}}: \textbf{(Question)} Was he abusive, tell me more.\\
    & \underline{\textit{seeker}}: I tried a lot but i couldn't forget him at all  \\
    & \underline{\textit{seeker}}: He was not abusive at all  \\
     \midrule
    Ground Truth & \textbf{(Question)} So what was the problem? \\
    \midrule
    GPT-4 & \textbf{(Affirmation and Reassurance)} I'm really sorry to hear that you're going through this. Breakups can be really tough, but remember, it's okay to grieve the relationship and it's okay to feel sad. It's a part of the healing process. You're stronger than you know. \\
    \cmidrule(lr){2-2}
    ChatGPT & \textbf{(Affirmation and Reassurance)}  It's okay to still feel hurt even if he wasn't abusive. Breakups are tough.\\
    \midrule
    Tulu & \textbf{(Affirmation and Reassurance)} You'll find another good person. I know it's hard, but it's very important to move on.\\
    \cmidrule(lr){2-2}
    LLaMA2-70B & \textbf{(Question)} What happened?\\
    \cmidrule(lr){2-2}
    Vicuna & \textbf{(Reflection of Feelings)} I can imagine how hard that must be for you. It sounds like you’re really hurting.\\
    \cmidrule(lr){2-2}
    Solar & \textbf{(Affirmation and Reassurance)} It's understandable that you're struggling with the breakup, but you've shown great resilience by acknowledging and expressing your feelings, which is an important step towards healing.\\
    \cmidrule(lr){2-2}
    Mistral & \textbf{(Affirmation and Reassurance)} That is completely understandable, it takes time to recover from a breakup.\\
    \cmidrule(lr){2-2}
    LLaMA2-7B & \textbf{(Question)} Did he ever abuse you?\\
     \bottomrule
\end{tabular}}
\caption{Example of the responses from LLMs in the \textit{Exploration} stage.}

\label{tab:case_llms_ques}
\end{table*}


==> tab_tex/case_study_llms_2.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l p{10cm}}
    \toprule
    Dialogue Background & The following is a conversation between a supporter and a seeker about fear regarding a/an job crisis. The seeker says "\textbf{I fear that I will not have a job next year, at the beginning of the year. My emotions are in survival mode and I do not want to do anything or buy anything from this fear.}" \\
    \midrule
    \multirow{23}{*}{
        \textbf{Dialogue Context}
    }
    & ... \\
    & \underline{\textit{seeker}}: I feel that I have not ideas. I feel like i have been thinking about a business idea for myself and family for some time now. I wonder how others decide on what to do\\
    & \underline{\textit{seeker}}: Like how to get that motivation in their head to start something really new \\
    & \underline{\textit{supporter}}: \textbf{(Providing Suggestions)} My suggestion would be to think what your local neighborhood needs - maybe it is lacking a cafe or a grocery store? \\
    & \underline{\textit{seeker}}: I know, i really want a niche company.. Something that no one has thought of, or is not yet in my community. \\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} Yes, I can identify with that. Motivation is hard - but think about your future job situation and your family. \\
    & \underline{\textit{seeker}}: I would love to do a zero waste company or store, since that is what I am really into. \\
    & \underline{\textit{seeker}}: Do you think it is hard to set up a business plan?\\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} That's a great idea! Green is the new way to go! I believe in you.\\
    & \underline{\textit{seeker}}: Oh Thank You! \\
    & \underline{\textit{supporter}}: \textbf{(Information)} I think it will take some hard work but you can do it. There are support for you from local governments. I think you should look into it. \\
    & \underline{\textit{supporter}}: \textbf{(Question)} How are you feeling now? \\
    & \underline{\textit{seeker}}: I think I will!\\
    & \underline{\textit{seeker}}: I actually feel motivated to do some research on this. \\
    & \underline{\textit{seeker}}: At least is has taken my mind off possibly not having a job \\
     \midrule
    Ground Truth & \textbf{(Affirmation and Reassurance)} That's great to hear! My suggestion is to always think positively. You can do this!\\
    \midrule
    GPT-4 & \textbf{(Affirmation and Reassurance)} That's wonderful to hear! Remember, taking the first step is often the hardest part. Keep going and don't give up.\\
    \cmidrule(lr){2-2}
    ChatGPT & \textbf{(Affirmation and Reassurance)} That's great to hear! Sometimes taking action is the best way to alleviate fear.\\
    \midrule
    Tulu &\textbf{(Affirmation and Reassurance)} I'm so glad to hear that. I think that it is the perfect distraction. You will be able to focus on building your future. \\
    \cmidrule(lr){2-2}
    LLaMA2-70B & \textbf{(Affirmation and Reassurance)} That is great to hear!\\
    \cmidrule(lr){2-2}
    Vicuna & \textbf{(Reflection of Feelings)} I understand how you feel, I've had similar fears too. But it's good to see you taking steps towards a solution. And it's great that you have a passion for the zero waste concept.\\
    \cmidrule(lr){2-2}
    Solar & \textbf{(Reflection of Feelings)} It's great to see that your emotions have shifted from fear to motivation. That is a positive change. Remember to take it one step at a time, and always know that you have support.\\
    \cmidrule(lr){2-2}
    Mistral & \textbf{(Affirmation and Reassurance)} It sounds like you have a lot of pain going on right now.\\
    \cmidrule(lr){2-2}
    LLaMA2-7B & \textbf{(Affirmation and Reassurance)} I believe in you!\\
     \bottomrule
\end{tabular}}
\caption{Example of the responses from LLMs in the \textit{Comforting} stage.}

\label{tab:case_llms_affirmation}
\end{table*}

==> tab_tex/case_study_llms_3.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{l p{10cm}}
    \toprule
    Dialogue Background & The following is a conversation between a supporter and a seeker about sadness regarding a/an ongoing depression. The seeker says "\textbf{I have a daughter who has decided to go live with her dad. I'm having a hard time with this. She is 16. And that's her decision. I'm fine with that part but I'm not fine with her not seeing me or spending time with me. 3 months age I grounded her and she's been upset with me ever since. She needed it though. She was getting out of hand. This is my baby girl. Her dad thinks everything is ok. like it is but I feel I have a right to see my daughter as well.}" \\
    \midrule
    \multirow{20}{*}{
        \textbf{Dialogue Context}
    }
    & ... \\
    & \underline{\textit{seeker}}: My daughter is 16 and got out of hand for a little while. I grounded her. And since that time, she has decided to move in with her dad. which is fine. But I've only gotten to see her once in 3 months. She don't want to see me.\\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} That's tough, I'm sorry. I don't have children of my own yet, but I remember being a teenager and having a similar phase. If it makes you feel any better, I eventually grew out of that phase and have a wonderful relationship with my parents now!\\
    & \underline{\textit{seeker}}: That's good. \\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} With the holidays coming up, maybe that's a good opportunity to reunite and spend some quality time with her?\\
    & \underline{\textit{seeker}}: By law though I don't think that my ex husband can keep her from me? I feel like I have a right to see my child. I have 4 kids altogether. My other 2 daughters are older and have already moved out and my son is still at home. I've dealt with teenagers and it's not easy but this is too extreme.\\
    & \underline{\textit{seeker}}: I asked about the holidays and she said she didn't know. It's gonna be hard not having her here.\\
    & \underline{\textit{supporter}}: \textbf{(Question)} Does she have a good relationship with her siblings? Maybe they can help convince her to spend some family time at home?\\
    & \underline{\textit{seeker}}: She did but not so great anymore. I sure hope so.\\
    & \underline{\textit{seeker}}: It's been hard on everybody. especially her little brother.\\
   
     \midrule
    Ground Truth & \textbf{(Providing Suggestions)} Maybe she just needs some time to decompress. Being a teenager is a stressful time, especially this year with everything with COVID. I'm hopeful that she will come out of this phase.\\
    \midrule
    GPT-4 & \textbf{(Providing Suggestions)} Perhaps you and her siblings can speak to her together. Express your feelings and let her know how much you all miss her. Sometimes, hearing from multiple people can have a greater impact.\\
    \cmidrule(lr){2-2}
    ChatGPT & \textbf{(Providing Suggestions)} Maybe you can try to plan some fun activities for the holidays that she would enjoy. It might help her feel more comfortable coming back home.\\
    \midrule
    Tulu & \textbf{(Affirmation and Reassurance)} That sounds difficult, especially for your son. I hope things get better for you and your family.\\
    \cmidrule(lr){2-2}
    LLaMA2-70B & \textbf{(Self-disclosure)} I can relate, I moved out of my parents' home at a very young age and that made it hard for me to spend time with them.\\
    \cmidrule(lr){2-2}
    Vicuna & \textbf{(Affirmation and Reassurance)} I can only imagine how difficult this is for you. It's great that you have a good relationship with your children, and I'm sure that will continue even if it's not always easy. %Just remember to take care of yourself too, it's important.
    \\
    \cmidrule(lr){2-2}
    Solar & \textbf{(Self-disclosure)} I understand how important it is to maintain family ties during difficult times. I had a similar experience with my own child, and it was challenging, but we eventually resolved the situation. %Keep the lines of communication open, and remember that your love and support will ultimately help your daughter realize the value of family.
    \\
    \cmidrule(lr){2-2}
    Mistral & \textbf{(Reflection of Feelings)} It takes a lot of courage to make a change and to start a new chapter in your life. I am happy that you are reaching out to me and that you are willing to take this step.\\
    \cmidrule(lr){2-2}
    LLaMA2-7B & \textbf{(Affirmation and Reassurance)} I'm so sorry to hear about your situation. I hope you feel better soon.\\
     \bottomrule
\end{tabular}}
\caption{Example of the responses from LLMs in the \textit{Action} stage.}

\label{tab:case_llms_information}
\end{table*}

==> tab_tex/case_study_method_1.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l p{10cm}}
    \toprule
    Dialogue Background & The following is a conversation between a supporter and a seeker about fear regarding a/an job crisis. The seeker says "\textbf{I am so scared of going out and finding a job due to Covid 19 but I need to work right now. my bills are piling up}" \\
    \midrule
    \multirow{18}{*}{
        \textbf{Dialogue Context}
    }
    & ... \\
    & \underline{\textit{seeker}}: I live with my grandmother and my mom who are both elderly or have underlying health conditions \\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} I understand. You are scared to put them in danger, correct? \\
    & \underline{\textit{seeker}}: Yes, I also don't want them to have to support me and my family either.\\ 
    & \underline{\textit{supporter}}: \textbf{(Reflection of Feelings)} With keeping your family in mind while trying to find a job have you considered looking for an online job? Just from chatting with you I can tell how much it stresses you out. \\
    & \underline{\textit{seeker}}: I have tried but it seems I am way out my league due to me working in Bars, cafes, and restaurants my entire life.\\
    & \underline{\textit{supporter}}: \textbf{(Providing Suggestions)} I understand I felt that way when trying to find new opportunities for myself. I kept looking and tried to apply the skills I learned to fit into the new requirements. Maybe a call representative. I assume from previous experience you have excellent customer service skills \\
    & \underline{\textit{seeker}}: Yes I actually do, I also have pretty good typing skills as well. \\
    & \underline{\textit{supporter}}: \textbf{(Information)} From that answer i believe that job could be a good fit! \\
    & \underline{\textit{seeker}}: Sure coud be. How did you know you could work online for a living? Is this a field you always worked in? \\
    \midrule
    Ground Truth & \textbf{(Self-disclosure)} With Covid I also lost my job. I looked online and it is currently a field I am pursuing. I don't do call center work but I do social media marketing all from the comfort of my home. \\
    \midrule
    ChatGPT 0-shot & \textbf{(Affirmation and Reassurance)} It's completely understandable that you're worried about putting your family at risk. You're being very considerate of their health and well-being. \\
    \midrule
    Direct Refine & \textbf{(Affirmation and Reassurance)} It's completely understandable that you're worried about putting your family at risk. You're being very considerate of their health and well-being. It's clear that you care deeply about their safety. \\
    \cmidrule(lr){2-2}
    Self-Refine & \textbf{(Affirmation and Reassurance)} It's completely understandable that you're worried about putting your family at risk. You're being very considerate of their health and well-being. It's clear that you want to make sure they're safe while also providing for your family. \\
    \cmidrule(lr){2-2}
    Emotional-CoT & \textbf{(Restatement or Paraphrasing)} It sounds like you are worried about finding a job that won't put your family at risk and also feeling unsure about your ability to adapt to online work due to your previous experience.\\
    \midrule
    w/ COMET & \textbf{(Self-disclosure)} No, I actually worked in a completely different field before transitioning to an online job. It took some time, but I found something that fits my skills and lifestyle. \\
    \cmidrule(lr){2-2}
    w/ Example Expansion & \textbf{(Self-disclosure)} I have worked in a variety of fields, but I found that my writing and communication skills translated well to online work. \\
    \cmidrule(lr){2-2}
    w/ Strategy Planner & \textbf{(Self-disclosure)} I actually have a friend who transitioned from working in a restaurant to working as a virtual assistant. It's definitely possible to make a change, and I think you have the skills to do it. \\
     \bottomrule
\end{tabular}}
\caption{Example of self-contact methods and external-contact methods on ChatGPT.}

\label{tab:case_method_compare}
\end{table*}

==> tab_tex/case_study_method_2.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l p{10cm}}
    \toprule
    Dialogue Background & The following is a conversation between a supporter and a seeker about depression regarding a/an ongoing depression. The seeker says "\textbf{I find it hard to get motivated, I suffer from low mood and don't know how to get out of this.}" \\
    \midrule
    \multirow{25}{*}{
        \textbf{Dialogue Context}
    }
    & ... \\
    & \underline{\textit{seeker}}: Yeah. I worry that I'll just keep feeling even more down and depressed. I'm really having a bad time and struggle to get out of bed to be honest. \\
    & \underline{\textit{supporter}}: \textbf{(Affirmation and Reassurance)} Firstly, you are not alone in feeling this way. Many people struggle with depression and it's good that you have reached out for help for this. \\
    & \underline{\textit{seeker}}:Any suggestions on what to do about it? \\ 
    & \underline{\textit{supporter}}: \textbf{(Information)} There are many reasons people have depression. It is a recognised medical condition and the good news is that there is help out there. The first step is recognizing the problem. \\
    & \underline{\textit{seeker}}: Ok well there is definitely a problem. \\
    & \underline{\textit{supporter}}: \textbf{(Question)} Have you spoken to friends and family about this? do they know how much you are struggling with it at the moment? \\
    & \underline{\textit{seeker}}: Ok well there is definitely a problem. \\
    & \underline{\textit{supporter}}: \textbf{(Providing Suggestions)} if people care about you then they will be happy to give you the time and listen to how you are feeling at the moment. I think it will be a really good move to speak to family or friends tell them how you are feeling and talk it through this might really help. \\
    & \underline{\textit{seeker}}: Yeah maybe. I suppose nobody really understands but I could at least speak to them about it. \\
    & \underline{\textit{supporter}}: \textbf{(Providing Suggestions)} everyone has problems and it is good to talk about them because a problem shared is a problem halved. It doesn't mean the problems will go away but it might help you understand them and then be able to deal with them better. \\
    & \underline{\textit{seeker}}: I don't want to feel like this anymore. I'm willing to at least give it a go. \\
    \midrule
    Ground Truth & \textbf{(Information)} I also think that it will be worse to get in touch with your doctor or a medical professional. these people are trained to deal with problems like yours and will be able to offer effective Solutions from a medical perspective. \\
    \midrule
    ChatGPT 0-shot & \textbf{(Affirmation and Reassurance)} It's great to hear that you're willing to give it a go. That shows strength and determination, and those are important qualities for working through depression. You're taking a positive step forward. \\
    \midrule
    Direct Refine & \textbf{(Affirmation and Reassurance)} Your willingness to give it a try is a strong and positive step forward. It shows that you have the strength and determination needed to work through depression. You're not alone in this, and there is hope for improvement. \\
    \cmidrule(lr){2-2}
    Self-Refine & \textbf{(Affirmation and Reassurance)} Your willingness to give it a go is truly commendable. It takes a lot of strength and determination to take this step, and I believe you have what it takes to work through this. You're moving in the right direction. \\
    \cmidrule(lr){2-2}
    Emotional-CoT & \textbf{(Reflection of Feelings)} It sounds like you are really struggling with your depression and feeling overwhelmed by it. It's important to acknowledge how difficult it is for you right now. \\
    \midrule
    w/ COMET & \textbf{(Affirmation and Reassurance)} It's really positive that you're willing to give it a go. That's a great first step in working towards feeling better. \\
    \cmidrule(lr){2-2}
    w/ Example Expansion & \textbf{(Affirmation and Reassurance)} That's a really positive step to take. I believe that with the right support and help, you can overcome this and start feeling better. \\
    \cmidrule(lr){2-2}
    w/ Strategy Planner & \textbf{(Information)} Have you considered seeking out networking opportunities to help rebuild your confidence and connections in the workforce? \textcolor{red}{(misalignment with \textit{Information})} \\
    \bottomrule
\end{tabular}} 
\caption{Example of misalignment between strategy and response in \textit{Strategy Planner} on ChatGPT.}
\label{tab:case_method_misalign}
\end{table*}


==> tab_tex/prompt_detail.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l p{10cm} p{4.5cm}}
    \toprule
    \textbf{Methods} & \textbf{Task Description} & \textbf{Postfix Prompt}\\ 
    \midrule
    Vanilla &  You are given a dialogue context between seeker and supporter. Your task is to make the next response based on the given dialogue context. & \#\#\# Model's response \#\#\#\\
    Direct-Refine & & \\
    Self-Refine & & \\
    w/ COMET & You are given a dialogue context between seeker and supporter, and a commonsense knowledge from external model. Your task is to generate a response for the supporter based on the dialogue context and commonsense knowledge, you should ignore the commonsense knowledge if it mislead the next response. Your role is to engage in a conversation as an emotional supporter, aiming to lower the intensity of the seeker's emotions. & \begin{tabular}{@{}l@{}}
          \#\#\# Commonsense knowledge \#\#\# \\
          $\{$comet$\}$ \\
          \#\#\#  Model's response \#\#\#
    \end{tabular}\\
    w/ Strategy Planner & & \\
    w/ Example Expansion & & \\
    \bottomrule
\end{tabular}
}
\caption{An example prompt for response generation.}

\label{tab:prompt_initial_2}
\end{table*}
